DiCA: A Hardware-Software Co-Design for Differential Checkpointing in Intermittently Powered Devices

Intermittently powered devices rely on opportunistic energy-harvesting to function, leading to recurrent power interruptions. This paper introduces DiCA, a proposal for a hardware/software co-design to create differential check-points in intermittent devices. DiCA leverages an affordable hardware module that simplifies the check-pointing process, reducing the check-point generation time and energy consumption. This hardware module continuously monitors volatile memory, efficiently tracking modifications and determining optimal check-point times. To minimize energy waste, the module dynamically estimates the energy required to create and store the check-point based on tracked memory modifications, triggering the check-pointing routine optimally via a nonmaskable interrupt. Experimental results show the cost-effectiveness and energy efficiency of DiCA, enabling extended application activity cycles in intermittently powered embedded devices.

==> pages/old-background.tex <==
\section{Background \& Literature Review}

% \red{talk about differencial between our solution and existing memory trackers}
% It is important to note that writing to FRAM in smaller sizes than the minimum block size can result in decreased performance and increased power consumption, as the controller may have to perform additional operations to read or write the data. Therefore, it is generally recommended to write to FRAM in block sizes that are equal to or greater than the minimum block size.


In this section, we provide a comprehensive background and literature review on checkpointing, intermittent computing, and memory tracking. 
% By examining the existing literature in these areas, we aim to identify the gaps and limitations that motivate the need for a novel checkpointing technique designed for intermittent devices.

\subsection{Checkpointing}

Checkpointing is a well-established technique used in computing systems to preserve the program state and to ensure fault tolerance during failure events. The checkpoint generation process involves saving the state of a running program on the device, including variables, registers, volatile memory and other relevant data, to a secondary storage known as a checkpoint.  The program can be restored to a previously saved checkpoint, minimizing data loss and enabling the system to continue execution from a known state. Checkpointing is implemented to provide resilience against power outages, software or hardware faults, or system crashes. [] 

The implementation of checkpoint techniques mitigates severe consequences of system or hardware failures that lead to loss of program state. Without checkpointing, the application would have to restart the execution causing the loss of intermediate results, wasted computational effort, and potential data corruption. Checkpointing provides a method to minimize the impact of failures and faults by restoring the program state to a saved stable state. 

Over the years, several checkpointing techniques have been developed, each with their own requirements and features. Checkpointing techniques are chosen based on the system, performance and memory considerations, hardware constraints and the types of failures that should be addressed. Traditional checkpointing methods save the entire state and data periodically, at regular intervals. This type of full checkpointing includes saving all variables, parameters, and data structures involved in the computation. For most applications, this is an inefficient model as values are inconsistently being modified, in addition to the high computation cost and the significant consumption of storage []. 

Differential checkpointing aims to increase effectiveness of checkpointing by selectively saving updated or modified information rather than the whole state. This technique helps to reduce the overhead and computational cost. This technique has been used in virtual machines and multi-processor operating systems [] for fault tolerance. Some implementations use specialized hardware such as memory management units (MMU) to support differential computation. 

% In database systems, checkpointing is implemented to ensure read consistency in with replicas, preventing transaction errors for example. For long, the ARIES ((Algorithm for Recovery and Isolation Exploiting Semantics) system has been used in databases, which performs fuzzy checkpointing []. Fuzzy checkpointing allows the normal application to continue executing during the checkpoint generation process. This reduces the overhead of full checkpointing but requires a stable storage medium and access to significant resources. Fuzzy checkpointing would not be possible on power-constrained devices with limited resources due to unpredictable availability. 


\subsection{Intermittent Computing}

Intermittent devices in the form of sensors and microcontrollers are emerging technologies in the IoT industry. They are cheaper, more eco-friendly than their battery-powered counterparts and can be deployed in the most remote places without requiring routine maintenance. These devices rely on power sources in the environment that are unreliable and the likelihood of energy exhaustion causing a shutdown mid-computation is high. Intermittent computing involves designing systems that can effectively operate and recover from power interruptions or supply variations. Challenges to intermittent computing include data loss, inconsistency during power interruptions, inefficient utilization of power and loss of program state []. 

The concept of checkpointing is implemented in these intermittent devices to preserve the state of the device prior to energy depletion and to resume operations at a later time when enough energy has been harvested. Much research into checkpoint techniques for intermittent computing has been conducted in the past decade. Power-aware algorithms and scheduling strategies could optimize system performance while considering the intermittent power supply [Hibernus, HarvOS, Mementos]. These techniques dynamically adapt the system's behavior, workload distribution, and resource allocation based on the available power and system requirements.  

This aspect of checkpointing for intermittent devices deals with the ‘when’ of checkpoint generation. Certain solutions trigger an interruption to the program based on the passing of a threshold, reacting by generating a checkpoint []. Other solutions employ a proactive approach using compile-time instrumentation to determine ideal checkpoint times []. However, these techniques can be resource-intensive, leading to research into providing intermittent devices with specialized hardware to alleviate the overhead. Recent research has considered non-volatile memory (NVM), such as flash memory or emerging NVM technologies, to store program state and data persistently. This approach allows for faster and more energy-efficient checkpointing and recovery mechanisms []. 


\subsection{Memory Tracking}


